A General Framework For Proving The Equivariant Strong Lottery Ticket Hypothesis

The Strong Lottery Ticket Hypothesis (SLTH) stipulates the existence of a subnetwork within a sufficiently overparameterized (dense) neural network that -- when initialized randomly and without any training -- achieves the accuracy of a fully trained target network. Recent works by Da Cunha et. al 2022; Burkholz 2022 demonstrate that the SLTH can be extended to translation equivariant networks -- i.e. CNNs -- with the same level of overparametrization as needed for the SLTs in dense networks. However, modern neural networks are capable of incorporating more than just translation symmetry, and developing general equivariant architectures such as rotation and permutation has been a powerful design principle. In this paper, we generalize the SLTH to functions that preserve the action of the group $G$ -- i.e. $G$-equivariant network -- and prove, with high probability, that one can approximate any $G$-equivariant network of fixed width and depth by pruning a randomly initialized overparametrized $G$-equivariant network to a $G$-equivariant subnetwork. We further prove that our prescribed overparametrization scheme is optimal and provides a lower bound on the number of effective parameters as a function of the error tolerance. We develop our theory for a large range of groups, including subgroups of the Euclidean $\text{E}(2)$ and Symmetric group $G \leq \mathcal{S}_n$ -- allowing us to find SLTs for MLPs, CNNs, $\text{E}(2)$-steerable CNNs, and permutation equivariant networks as specific instantiations of our unified framework. Empirically, we verify our theory by pruning overparametrized $\text{E}(2)$-steerable CNNs, $k$-order GNNs, and message passing GNNs to match the performance of trained target networks.

==> Burkhlotz_work.tex <==
 We note that our proof can then be extended trivially to this different setting by leveraging again the fact that the identity is equivariant. The result is then exactly what we obtain when one takes $G$ the group of translations in Theorem \ref{thm:main_approx_network}.

==> old_background.tex <==
\subsection{Equivariant Networks}
\label{Equivariant_Networks}
In this section we briefly review the necessary facts regarding equivariance and invariance to certain pre-specified symmetries. First, recall the main definition for equivariance:
\begin{definition}
Let $\mathcal{X}$ and $\mathcal{Y}$ be two sets with an action of a group $G$. A map $\phi: \mathcal{X} \to \mathcal{Y}$ is called $G$-equivariant, if it respects the action, i.e., $g\cdot \phi(x) = \phi(g \cdot x), \forall g\in G$ and $x \in \mathcal{X}$.  A map $\psi: \mathcal{X} \to \mathcal{Y}$ is called $G$-invariant, if $\psi(x) = \psi(g \cdot x), \forall g\in G$ and $x \in \mathcal{X}$.
\end{definition}
In this paper, we will always take sets $\mathcal{X}, \mathcal{Y}$ to be real vector spaces. Thus, to build an equivariant network it is sufficient to use a $G$-equivariant non-linearity (e.g. pointwise ReLU) and to take each layer, $\phi_i$,  $\Phi = \phi_l \circ \phi_{l-1} \circ \dots \phi_1$ to be $G$-equivariant as a composition of equivariant function is itself equivariant. An invariant network can easily be built from an equivariant net by simply utilizing an invariant function as the output on an equivariant net---i.e. $\Psi = \psi \circ \phi_{l} \circ \dots \phi_1$. To construct equivariant maps as layers in $G$-equivariant network we must first specify the group and how it \emph{acts} on the underlying (feature) space, which we outline below for our two main groups of interest.  

\xhdr{$\text{E}(2)$-equivariant nets}
The Euclidean group $\text{E}(2)$ is the group of isometries of the plane $\mathbb{R}^2$ and is defined as the semi-direct product between the translation and orthogonal groups of two dimensions $ (\mathbb{R}^2, + ) \rtimes \text{O}(2)$. The most general method to build equivariant networks for $\text{E}(2)$ is in the framework of 
steerable $G$-CNN's which represent the input $x$, as a signal over a homogenous space (a manifold where $G$ acts transitively) and design convolutional filters that are \textit{steerable} with respect to the action of the group \cite{cohen2016steerable,cohen2018intertwiners,weiler2018learning}. Concretely, steerable feature fields associate a $c$-dimensional feature vector to each point in a base space $f: \mathbb{R}^2 \to \mathbb{R}^c$ which identifies the appropriate transformation law under the action of a group.
For example, a gray scale image $x$ can be thought of as a scalar field $s: \mathbb{R}^2 \to \mathbb{R}$ over the 2D-plane where at each pixel co-ordinate we associate an intensity value. Now an action of $\text{E}(2)$ by some $(tg) \in  (\mathbb{R}^2, + ) \rtimes \text{O}(2)$ on the scalar field $s$ results in moving a pixel to its new position: $s(x) \mapsto s((tg)^{-1}x) = s(g^{-1}(x-t))$. 


To understand how these fields transform $f: \mathbb{R}^2 \to \mathbb{R}^c$, we must specify a group representation $\rho: G \to GL(\mathbb{R}^c)$, which  itself is a group and satisfies $\rho(g_1g_2) = \rho(g_1)\rho(g_2)$ with the group operation being ordinary matrix multiplication, e.g.  2D-rotations  are $2 \times 2$ rotation matrices. Thus, feature fields in steerable $\text{E}(2)$-CNNs transform according to their \emph{induced representation} $\left[\Ind^{(\mathbb{R}^{2}\rtimes G)}_{G}\rho\right]$,
\begin{equation}
    f(x) \rightarrow \left(\left [\Ind^{(\mathbb{R}^{2}\rtimes G)}_{G}\rho \right ](tg) \cdot f \right)(x) := \rho(g) \cdot f(g^{-1}(x-t)).
\end{equation}
Equipped with this feature spaces in steerable $G$-CNNs are represented as stacks of feature fields $f = \bigoplus_i f_i$ with each field $f_i$ being associated its own representation type $\rho_i$ which results in a block diagonal direct sum representation over the entire feature space. Clearly, an input RGB image--a scalar field---transforms to the \emph{trivial representation} $\rho(g) = 1\,,\; \forall g \in G$, but intermediate layers may transform according to other representation types such as regular or irreducible. As proven in \citet{cohen2019general}, any equivariant linear map between steerable feature spaces transforming under $\rho_{in}$ and $\rho_{out}$ must be a group convolution with $G$-steerable kernels $\pi: \mathbb{R}^{c_{out}} \times \mathbb{R}^{c_{in}}$ which satisfy the following equivariance constraint: $\pi(gx) = \rho_{out}(g)\pi(x)\rho_{in}(g^{-1}) \ \forall g \in G, x \in \mathbb{R}^2$. %In section \ref{}, we will seek to approximate a group convolution using two overparametrized group convolutions. 




\xhdr{$\gS_n$-equivariant nets} The symmetric group $\gS_n$ consists of all permutations that can enacted on a set of cardinality $|n|$. It's action on a vector $x \in \mathbb{R}^n$ consists of a permutation of the dimensions defined as: $g \cdot x = (x_{g^{-1}(1)}, \dots, x_{g^{-1}(n)}), g \in G \leq \gS_n$. The action of $\gS_n$ on a tensor $\tX \in \mathbb{R}^{n^k \times a}$ is defined analogously and corresponds to permuting all but last index: $(g \cdot \tX)_{i_1, \dots, i_k, j} = (\tX_{g^{-1}(i_1)}, \dots g^{-1}(i_k), j), \forall g \in G$. Any general linear permutation equivariant map $L: \mathbb{R}^{n^{k} \times a} \rightarrow \mathbb{R}^{n^{l} \times b}$ \cite{maron2018invariant}, must satisfy the following fixed point equation:
\begin{equation}
    \label{permutation constraint}
    \mathbf{P^{\otimes(k+l)} \Vect(L)=L}
\end{equation}
where $\mathbf{P^{\otimes(k+l)}}$ is the $(k+l)$ is the Kroenecker power of the action on a permutation matrix $\mathbf{P}$.% which represents the action of a permutation matrix $\mathbf{P}$.
